EncodeNet: A Framework for Boosting DNN Accuracy with Entropy-driven Generalized Converting Autoencoder

Image classification is a fundamental task in computer vision, and the quest to enhance DNN accuracy without inflating model size or latency remains a pressing concern. We make a couple of advances in this regard, leading to a novel EncodeNet design and training framework. The first advancement involves Converting Autoencoders, a novel approach that transforms images into an easy-to-classify image of its class. Our prior work that applied the Converting Autoencoder and a simple classifier in tandem achieved moderate accuracy over simple datasets, such as MNIST and FMNIST. However, on more complex datasets like CIFAR-10, the Converting Autoencoder has a large reconstruction loss, making it unsuitable for enhancing DNN accuracy. To address these limitations, we generalize the design of Converting Autoencoders by leveraging a larger class of DNNs, those with architectures comprising feature extraction layers followed by classification layers. We incorporate a generalized algorithmic design of the Converting Autoencoder and intraclass clustering to identify representative images, leading to optimized image feature learning. Next, we demonstrate the effectiveness of our EncodeNet design and training framework, improving the accuracy of well-trained baseline DNNs while maintaining the overall model size. EncodeNet's building blocks comprise the trained encoder from our generalized Converting Autoencoders transferring knowledge to a lightweight classifier network - also extracted from the baseline DNN. Our experimental results demonstrate that EncodeNet improves the accuracy of VGG16 from 92.64% to 94.05% on CIFAR-10 and RestNet20 from 74.56% to 76.04% on CIFAR-100. It outperforms state-of-the-art techniques that rely on knowledge distillation and attention mechanisms, delivering higher accuracy for models of comparable size.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/5_Result.tex <==
\section{Results} \label{results}
This section discusses the comprehensive evaluation of our work with other competing techniques. We compare widely used methods for Knowledge Distillation and attention mechanisms across CIFAR-10 and CIFAR-100 datasets.
We present the results demonstrating the enhanced accuracy achieved for the baseline deep neural network (DNN) as a result of our framework.

\subsection{Improvement of Baseline DNN}
Table~\ref{tab:Improved_baselines} presents comprehensive results illustrating the improvement in accuracy for the baseline network achieved through the robust training of our framework. For comparison, we evaluated various derivatives of two types of networks: VGG~\cite{VGG16} and ResNet~\cite{ResNet}. VGG8 exhibited an increase in accuracy of 1.89\% and 3.2\% for the Cifar10 and Cifar100 datasets, respectively. VGG16 demonstrated an improvement of approximately 1.8\% to 2.0\% in accuracy over the baseline due to EncodeNet. Similarly, for different derivatives of ResNet, the accuracy gain was approximately 1-2\%.  

% \subsection{Comparison with Pooling Schemes}
% We compare various types of pooling operations to highlight the improvement in accuracy. Several pooling schemes have been proposed to enhance the accuracy of baselines without requiring additional parameters. We compared four widely used pooling techniques: Max Pooling~\cite{Ranzato2007SparseFL}, Mixed Pooling~\cite{Yu2014MixedPF}, and Accept-Reject Pooling~\cite{Accept_Reject_pooling}, which were trained on ResNet-20 with the CIFAR-10 dataset. The results indicate that our method outperforms other baselines in enhancing the baseline classification accuracy.


\subsection{Comparison with Knowledge Distillation Techniques}
To further evaluate our work, we compared it with existing knowledge techniques: KD (Knowledge Distillation), RKD (Relational Knowledge Distillation), FitNet, and FT (Factor Transfer). Results on the CIFAR-100 dataset indicate that our approach exhibits superior performance for both ResNet and VGG networks. We employed two sets of teacher-student models: one with ResNet-110 as the teacher and ResNet-32 as the student, and the other with VGG16 as the teacher and VGG8 as the student. The results demonstrate that our method outperforms other knowledge distillation techniques.


\subsection{Comparison with Attention Mechanisms}
We also compared EncodeNet with existing attention mechanism techniques: Squeeze-and-Excitation Networks (SE) ~\cite{hu2018squeeze}, Bottleneck Attention Module (BAM)~\cite{park2018bam} , Convolutional block attention module (CBAM) \cite{woo2018cbam} and Global attention mechanism (GAM) \cite{Liu2021GlobalAM}. In table \ref{table:attention_mechanism}, we observe that our framework can increase the accuracy of baseline DNN without increasing the parameters and model sizes, whereas most attention mechanism frameworks require substantial additional parameters. Global attention Mechanism (GAM) ~\cite{Liu2021GlobalAM} shows more improvement in classification accuracy, but a significant number of parameters need to be added to the baseline compared to other techniques.


\begin{comment}

\subsection{Comparison with Model Compression Methods}

We evaluate our framework with existing pruning techniques. Tables \ref{tab:Comparison_Cifar10_pruning} and \ref{tab:Comparison_Cifar100_pruning} present comparisons with baseline networks and other pruned method, as well as a comparison of parameter counts across the CIFAR-10 and CIFAR-100 datasets. For CIFAR-10, although our accuracy experiences a 1\% decrease compared to our competitive pruned methods, we achieve a significantly higher level of pruning for the baseline, approximately double that of the competitive method. For CIFAR100, our methods demonstrate superiority over other techniques both in terms of accuracy and pruned ratio. 
In this comparison, we initially begin with lightweight DNNs characterized by a small parameter count and aim to enhance these lightweight models to achieve similar accuracy levels as baseline or pruned larger models.

\end{comment}



\subsection{Ablation Studies}
\begin{table}[htb]
  \caption{Ablation studies on Cifar10}
  \label{tab:Ablation Studies}
  \centering
  \begin{tabular}{lcccc}
    \toprule
    Architecture  & Parameters       & Accuracy ($\%$)  \\
    \midrule

    ResNet 18 (Baseline) & 0.19 M  & 91.12 \\
    ResNet 18 + Intraclass Clustering & 0.19 M  & 92.87 \\
    ResNet 18 + Without Intraclass clustering & 0.19 M & 92.11   \\
    ResNet 18 + Same Image & 0.19 M & 89.26\\
    ResNet 18 + Representative Image & 0.19 M & 92.87\\
    \hline
  \end{tabular}
\end{table}
%We perform ablation studies on Cifar10 utilizing ResNet18. Table ~\ref{tab:Ablation Studies} illustrates the outcomes for Cifar10 with ResNet18 as a reference point. Our framework was assessed to gauge the effects of various methods implemented on EncodeNet. The table presents classification accuracy results with and without intraclass clustering, conversion to the same image, and representative images. Even though we observed intraclass clustering reduces the reconstruction error for the autoencoder in the final classification, it shows a minimal effect in improving classification accuracy.


We conducted ablation studies on Cifar10 using ResNet18. Table ~\ref{tab:Ablation Studies} depicts the results for Cifar10 with ResNet18 as a baseline. Our evaluation aimed to assess the impact of different methods applied to EncodeNet. The table displays classification accuracy results with and without intraclass clustering, conversion to the same image, and representative images. Although intraclass clustering was observed to reduce the autoencoder's reconstruction error, its effect on improving classification accuracy was minimal. On the contrary, when the target map is chosen as the representative image, as opposed to the same image, a noticeable improvement in accuracy was observed.














